Emerging Thermal-Metabolic Control of Phytoplankton Annual Cycles: Extending the Critical Depth Hypothesis

While the Critical Depth Hypothesis (CDH) established physical mixing and light availability as primary drivers of phytoplankton annual cycle, global thermal restructuring requires expanding this paradigm to incorporate temperature-dependent biological kinetics. We introduce a non-autonomous framework that extends the CDH into a temperature-dependent paradigm. By analyzing invasion dynamics at the boundary of extinction, we derive the critical nutrient saturation($\gamma$crit) as a structural threshold for population persistence across annual cycles. Applied to end-of-the-century projections from the GFDL-ESM4 model under a high-emission scenario (SSP5-8.5), our framework identifies an emerging thermal-metabolic control, which increasingly displaces regions where seasonal dynamics were historically governed by physical mixing. Relevance to Life Sciences. Disentangling the primary drivers of phytoplankton annual cycles is essential for understanding ecosystems under climate change. Our analysis extends CDH by demonstrating that thermal metabolism modifies the baseline required for annual population recovery. Projections under high-emission scenarios reveal that anthropogenic forcing alters this balance, shifting global phytoplankton driver control from physical mixing to thermal-metabolic. However, this transition is not homogeneous: the North Atlantic Subpolar Gyre serves as a mixing-driven anomaly where deep mixing dynamics and regional thermal stasis maintain historical control. By evaluating stability directly from model outputs, this methodology provides a computationally efficient diagnostic to map driver hierarchies across Earth System Models. Mathematical Content. We model seasonal ecosystem dynamics using a non-autonomous NPZ-t framework forced by periodic functions of temperature, light, and mixed layer depth. Linearizing around the extinction equilibrium E0 decouples the system into a diagonal periodic structure. The Floquet multiplier $\rho$P yields the annual invasion growth rate $\lambda$P , we prove that $\lambda$P > 0 is a sharp condition for uniform persistence (Theorem 2.2). Isolating the threshold condition $\lambda$P = 0 yields the definition of the critical nutrient saturation ratio, $\gamma$crit. A first-order Taylor sensitivity decomposition of $\gamma$crit allow us to assess the role of environmental anomalies for temperature ($\Delta$T ), mixing ($\Delta$H), and light amplitude ($\Delta$I) on phytoplankton annual cycles.

==> habitat_table.tex <==
\begin{table}[htbp]
    \centering
    \caption{Global area and ocean coverage of phytoplankton persistence regimes under the GFDL-ESM4 SSP5-8.5 projection (2015--2100).}
    \label{tab:habitat_stats_gfdl}
    \begin{tabular}{l c c}
    \toprule
    \textbf{Ecological Regime / Habitat} & \textbf{Area ($10^6$ km$^2$)} & \textbf{Ocean Coverage (\%)} \\
    \midrule
    Stable Viability & \GFDLStableViabilityArea & \GFDLStableViabilityPerc \\
    Stable Restriction & \GFDLStableRestrictionArea & \GFDLStableRestrictionPerc \\
    Habitat Expansion & \GFDLHabitatExpansionArea & \GFDLHabitatExpansionPerc \\
    Habitat Contraction & \GFDLHabitatContractionArea & \GFDLHabitatContractionPerc \\
    Ice-Free Viability & \GFDLIceFreeViabilityArea & \GFDLIceFreeViabilityPerc \\
    Ice-Free Restriction & \GFDLIceFreeRestrictionArea & \GFDLIceFreeRestrictionPerc \\
    \bottomrule
    \end{tabular}
\end{table}
